Statistical extraction of process zones and representative subspaces in fracture of random composite

We propose to identify process zones in heterogeneous materials by tailored statistical tools. The process zone is redefined as the part of the structure where the random process cannot be correctly approximated in a low-dimensional deterministic space. Such a low-dimensional space is obtained by a spectral analysis performed on pre-computed solution samples. A greedy algorithm is proposed to identify both process zone and low-dimensional representative subspace for the solution in the complementary region. In addition to the novelty of the tools proposed in this paper for the analysis of localised phenomena, we show that the reduced space generated by the method is a valid basis for the construction of a reduced order model.

==> PODOld.tex <==



\subsection{Proper orthogonal decomposition (POD)}

The Proper orthogonal Decomposition (POD) is a classical transform \cite{pearson1901,hotelling1933,sirovich1987} that aims at searching for an optimal expansion of the time evolution of a vector $\dispdiscr: \ \mathcal{T}^{h} \rightarrow \mathbb{R}^{n_u} $ (vector of nodal values of the displacement field in our case) as a sum of products of space vectors weighted by time functions. In this respect, the POD is based on the method of separation of variables (space and time in this context). We will denote by $\mathcal{V}^{h}$ the set of functions of time $t \in \mathcal{T}^{h}$ with values in $\mathbb{R}^{n_u}$. The POD looks for a function $\bar{\dispdiscr} \in \mathcal{V}^{h}$ in the form
\begin{equation}
\label{eq:SepVariables}
\begin{array}{rcl}
\displaystyle \bar{\dispdiscr}  : \quad \mathcal{T}^h  & \displaystyle \rightarrow & \mathbb{R}^{n_u}
\\ \displaystyle
\displaystyle t & \displaystyle \mapsto & \displaystyle \sum_{i=1}^{n_c} \V{\mathbf{C}}_i \, \alpha_i(t)  \, ,
\end{array}
\end{equation}
For all $i \in \llbracket 1, n_c \rrbracket$, $(\V{\mathbf{C}}_i \in \mathbb{R}^{n_u}$ is a so-called space vectors, while $\alpha_i \in \mathcal{F}({\mathcal{T}^{h}})$ is the associated time weight function.  $n_c \leq n_u$ is the order of the expansion. The POD transform minimises a distance $d_{\mathcal{V}^{h}}(\dispdiscr,\bar{\dispdiscr})$ between the expansion and the exact solution. The definition of this distance requires to introduce the natural inner product $<. \, , \, .>_{\mathcal{V}}$ in $\mathcal{V}^{h}$, and its associated norm $\| \, . \, \|_{\mathcal{V}^{h}}$ defined by
\begin{equation}
\begin{array}{l}
\displaystyle <\V{\mathbf{X}},\V{\mathbf{Y}}>_{\mathcal{V}^{h}} = \sum_{t \in \mathcal{T}^{h}} \V{\mathbf{X}}(t)^T \V{\mathbf{Y}}(t) 
\\
\displaystyle  \| \V{\mathbf{X}} \|_{\mathcal{V}^h} = <\V{\mathbf{X}},\V{\mathbf{X}}>_{\mathcal{V}^h}^\frac{1}{2}
= \left( \sum_{t \in \mathcal{T}^{h}} \| \X(t) \|^2_2 \right)^\frac{1}{2}
\, ,
\end{array}
\end{equation}
where $\V{\mathbf{X}}$ and $\V{\mathbf{Y}}$ are arbitrary elements of ${\mathcal{V}^{h}}$.
Let us introduce the matrix notation $\displaystyle \sum_{i=1}^{n_c} \V{\mathbf{C}}_i \, \alpha_i(t) = \basereduc \, \coeffreduc(t)$, for all $t \in  \mathcal{T}^h$, where the columns of operator $\basereduc \in \mathbb{R}^{n_u \times n_c}$ are the space vectors $\left( \V{\mathbf{C}}_i \right)_{i \in \llbracket 1, n_c \rrbracket}$, and $\coeffreduc$ is the column vector of the time functions $\left( \alpha_i \right)_{i \in \llbracket 1, n_c \rrbracket}$. With these compact notations, the POD looks for an optimal decomposition \eqref{eq:SepVariables} minimising metric
\begin{equation}
\label{eq:MetricPOD}
d_{\mathcal{V}^h}(\dispdiscr,\bar{\dispdiscr}) = \| \dispdiscr - \bar{\dispdiscr} \|_{\mathcal{V}^h}^2 \, ,
\end{equation}
under the constraint of orthonormality of the space vectors. Therefore, assuming that the exact solution $\dispdiscr$ is known, we look for the minimum of functional
\begin{equation}
\begin{array}{rcl}
\label{eq:MetricPOD2}
\bar{J}: \mathbb{R}^{n_u \times n_c} \times \left( \mathcal{F}(\mathcal{T}^h) \right)^{n_c} & \rightarrow & \mathbb{R} \\ 
(\basereduc,\coeffreduc) & \mapsto & d_{\mathcal{V}^h}(\dispdiscr, \bar{\dispdiscr} )
\end{array}
\end{equation}
under the constraint:
\begin{equation}
\label{eq:orthonorm}
\basereduc^T \basereduc = \M{\mathbf{I}}_d \, .
\end{equation}

The solution to optimisation problem (\ref{eq:MetricPOD2},\ref{eq:orthonorm}) requires the introduction of the POD ``correlation'' operator
\begin{equation}
\M{\mathbf{H}} = \sum_{t \in \mathcal{T}^h} \dispdiscr(t) \, \dispdiscr(t)^T \, .
\end{equation}
A global minimiser of functional $\bar{J}(\basereduc,\coeffreduc)$ is the following POD expansion:
\begin{itemize}
\item the time functions are such that $\coeffreduc(t) =  \basereduc^T  \, \dispdiscr(t) $, for all $t \in  \mathcal{T}^h$, which implies that decomposition $\bar{\dispdiscr}(t)=\basereduc \, \basereduc^T \dispdiscr(t)$ is the orthogonal projection of ${\dispdiscr}(t)$ onto $\textrm{Im}(\basereduc)$
\item the spacial modes $\left( \V{\mathbf{C}}_i \right)_{i \in \llbracket 1, n_c \rrbracket}$ are the eigenvectors of $\M{\mathbf{H}}$ associated to its largest $n_c$ eigenvalues $(\lambda_i)_{i \in \llbracket 1, n_c \rrbracket}$ ($\M{\mathbf{H}}$ has $n_u$ eigenvalues $(\lambda_i)_{i \in \llbracket 1, n_u \rrbracket}$ that are real and non-negative as $\M{\mathbf{H}}$ is real and symmetric)
\end{itemize}

The approximation error (i.e. the error due to the truncation of the expansion at order $n_c$) for a proper orthogonal decomposition $\bar{\dispdiscr}$ of $\dispdiscr$ is
\begin{equation}
\bar{J}(\basereduc , \coeffreduc) = \sum_{i=n_c+1}^{n_u} \lambda_i \, .
\end{equation}

For the POD transform to be useful in practice, the error of the decomposition should decrease quickly with order $n_c$. In other words, the space state of the solution in time $\dispdiscr$ should be well-approximated in a low-dimensional manifold $\textrm{Im}(\basereduc)$ of $\mathbb{R}^{n_u}$. In figure \ref{fig:PODconv}, the square root of the truncation error $\bar{J}(\basereduc , \coeffreduc)$ normalised by $\displaystyle \left(   \sum_{t \in \mathcal{T}^{h}} \| \dispdiscr(t) \|^2_2 \right)^\frac{1}{2} $ is plotted as a function of $n_c$, for one realisation  of the stochastic problem of fracture (see figure \ref{fig:RandomCracks}, top). One can observe that the time evolution, comprising 50 time successive time solutions, is well approximated by a POD expansion of order 5, for which the normalised truncation error is below $10^{-3}$. In other words, the solution of the problem can be represented with an acceptable degree of accuracy in a space $\textrm{Im}(\basereduc)$ of dimension 5.

 \begin{figure}[htb]
        \centering
        \includegraphics[width=0.6\linewidth]{figures/PODconv.pdf}
        \caption{Definition of the lattice problem.}
        \label{fig:PODconv}
 \end{figure}

The POD can be extended to parametric problem problems by replacing the time dependant weight functions by parameter dependant time functions in the afford derivations, and modifying the POD metric accordingly. In the present case of problems of evolution in random structures, we similarly look for weight functions depending on two variables: time and stochastic realisation. We define the time/stochastic space over which the solution is expanded by $\mathcal{P} = \mathcal{T}^{h} \times \Theta$. Applying the previous methodology, The POD in $\mathcal{P}$ comes down to the search of a projection of the exact solution $\dispdiscr \in \mathcal{W}^h$ (space of functions of $\mathcal{P}$ with values in $\mathbb{R}^{n_u}$) into a deterministic space $\textrm{Im}(\basereduc)$ of dimension $n_c$
\begin{equation}
\begin{array}{rcl}
\displaystyle \bar{\dispdiscr}  : \quad \mathcal{P}   & \displaystyle \rightarrow & \mathbb{R}^{n_u}
\\ \displaystyle
\displaystyle (t,\mu) & \displaystyle \mapsto & \displaystyle  \basereduc \,  \basereduc^T  \dispdiscr(t,\mu)  \, ,
\end{array}
\end{equation}
such that the following functional is minimised:
\begin{equation}
\begin{array}{rcl}
\label{eq:MetricPOD2}
J: \mathbb{R}^{n_u \times n_c} & \rightarrow & \mathbb{R} \\ 
\basereduc & \mapsto & \displaystyle \sum_{(t,\mu) \in \mathcal{P}} \| \dispdiscr (t,\mu)- \bar{\dispdiscr}(t,\mu)   \|_2^2
\end{array}
\end{equation}
As for the case of the POD in time, a reduced basis $(\V{\mathbf{C}}_i)_{i \in \llbracket 1 , n_c \rrbracket}$ of rank $n_c$ that minimises the above functional is composed of the eigenvectors of $\displaystyle \M{\mathbf{H}} = \sum_{(t,\mu) \in \mathcal{P}} \dispdiscr(t) \, \dispdiscr(t)^T $ associated to its $n_c$ largest eigenvalues $(\lambda_i)_{i \in \llbracket 1, n_c \rrbracket}$. The associated normalised error estimate reads:
\begin{equation}
%\begin{array}{ll}
\displaystyle  \nu  \displaystyle  
 = \left( \frac{\displaystyle J(\basereduc)}{\displaystyle \sum_{(t,\mu) \in \mathcal{P}} \| \dispdiscr(t,\mu) \|_2^2} \right)^{\frac{1}{2}} = \left( \frac{\displaystyle\sum_{i=n_c+1}^{n_u} \lambda_i}{\displaystyle \sum_{i=1}^{n_u} \lambda_i}   \right)^{\frac{1}{2}}  \, .
 %\end{array}
\end{equation}

The POD transform hence requires the knowledge of the time evolution of the solution over all possible outcomes of the random distribution, and, as such, can only be used for \textit{a posteriori} analysis and compression of data. In our case, obtaining the exact solution over all possible outcomes is not tractable. Instead, classical approaches for parametrised (or stochastic) problem propose to compute the exact solution corresponding to a limited number of parameter values (or random outcomes), and reuse these solutions to construct a relevant approximation of $\dispdiscr$ over the full parameter space. This can be achieved by applying the snapshot methodology, first described in \cite{sirovich1987}.


\subsection{Snapshot Proper orthogonal decomposition for stochastic evolution}

We directly expose the idea of the snapshot POD in the case of stochastic problems of evolution. We look for a POD-type decomposition $\bar{\dispdiscr}^s$ of solution $\dispdiscr$ that approximates $\bar{\dispdiscr}$ but only requires the knowledge of a set of pre-computed samples $\left\{ \dispdiscr(t,\mu) \right\}_{ \, (t,\mu) \in  \mathcal{T}^h \times \Theta^{s} } $.
%\begin{equation}
%\begin{array}{rcl}
 %\V{\mathbf{\mathbf{S}}}: \quad \mathcal{T}^h \times \Theta^{s} & \rightarrow & \mathbb{R}^{n_u} \\
  %(t,\mu) & \mapsto & \V{\mathbf{\mathbf{U}}}(t,\mu)
 %\end{array} \, ,
% \end{equation}
$\Theta^{s} $ is the subset of $\Theta$ corresponding to the random distribution of the samples. Let us define for simplicity $\mathcal{P}^s=\mathcal{T}^h \times \Theta^{s} $.  The snapshot POD expansion of $\dispdiscr$ reads
\begin{equation}
\label{eq:SepVariablesDiscrTime2}
\begin{array}{rcl}
\displaystyle \bar{\dispdiscr}^s  : \quad \mathcal{P}^s   & \displaystyle \rightarrow & \mathbb{R}^{n_u}
\\ \displaystyle
\displaystyle (t,\mu) & \displaystyle \mapsto & \displaystyle  \basereduc^s \,  {\basereduc^s}^T  \dispdiscr(t,\mu)  \, ,
\end{array}
\end{equation}
%Expansion $\bar{\V{\mathbf{\mathbf{S}}}}$ minimises a distance $d_{\mathcal{V}^h}(\V{\mathbf{\mathbf{S}}},\bar{\V{\mathbf{\mathbf{S}}}})$ defined in the space $\mathcal{V}^h$ 
 %of functions of $\tilde{\mathcal{P}}^h$ with values in $\mathbb{R}^{n_u}$.

%It has been very successful in the past years as it permits to provide an approximation of a Proper Orthogonal Decomposition without knowing the full solution $\dispdiscr$ \textit{a priori}. The principle is to work with a discrete set of solution samples, $\M{\mathbf{\mathbf{S}}} = \begin{pmatrix}
%\dispdiscr(t_1,1) & \dispdiscr(t_2,1) & ... & \dispdiscr(t_{n_t},n_\mu)
%\end{pmatrix}$ in the context of our problem of stochastic fracture mechanics, instead of the solution over the complete product space $\mathcal{V}$. 

%The Global POD still decompose the solution as a sum of product of functions of two separate sets  variables, whilst working with parameters evolving in more than one dimension. In our case, this means that the time and randomness dependency are treated indifferently.

%In our context, the Snapshot POD looks for a decomposition of $\bar{\V{\mathbf{\mathbf{S}}}} \in \mathcal{V}^h$ of $\V{\mathbf{\mathbf{S}}} \in \mathcal{V}^h$ under the form:
%\begin{equation}
%\label{eq:SepVariablesDiscr}
%\begin{array}{rcl}
%\displaystyle \bar{\V{\mathbf{\mathbf{S}}}}  : \quad \tilde{\mathcal{P}}^h & \displaystyle %\rightarrow & \displaystyle \mathbb{R}^{n} 
%\\ \displaystyle
%\displaystyle \bar{\V{\mathbf{\mathbf{S}}}}(t_n,\mu) & \displaystyle = & \displaystyle %\sum_{i=1}^{n_C} \V{\mathbf{C}}_i \, \alpha_i(t_n,\mu)  \, ,
%\end{array}
%\end{equation}

The reduced basis $\basereduc^s$ is found by minimisation of a functional $J^s$, which measures the distance between the exact solution samples and their orthogonal projection onto $\textrm{Im}(\basereduc)$:
\begin{equation}
\label{eq:snapmetric}
J^s(\basereduc) = \sum_{(t,\mu) \in \mathcal{P}^s} \| \dispdiscr(t,\mu) - \bar{\dispdiscr}^s(t,\mu) \|_2^2 \, ,
\end{equation}
The constraint  \eqref{eq:orthonorm} of orthonormality of the space vectors is enforced in the minimisation process. 
%In \eqref{eq:snapmetric}, function $\V{\bm{\epsilon}} \in \mathcal{V}$ is defined by $\V{\bm{\epsilon}}(t,\mu) = \dispdiscr(t,\mu) - \bar{\dispdiscr}(t,\mu)$ for all $(t,\mu) \in \tilde{\mathcal{P}}$. %
%It can be seen as a quadrature integration rule for \eqref{eq:MetricPOD}, with unitary weights. 
A minimiser of this problem is obtained when reduced basis $\left( \V{\mathbf{C}}_i \right)_{i \in \llbracket 1, n_c \rrbracket}$ is composed of the eigenvectors of $\displaystyle \M{\mathbf{H}}^s = \sum_{(t,\mu) \in \tilde{\mathcal{P}}^s} \dispdiscr(t,\mu) \,\dispdiscr(t,\mu)^T$ associated to its largest $n_c$ eigenvalues $(\lambda_i^s)_{i \in \llbracket 1, n_c \rrbracket}$.

Let us define the normalised  truncation error for the Snapshot POD of order $n_c$
\begin{equation}
%\begin{array}{ll}
\displaystyle  \nu^s  \displaystyle  
 = \left( \frac{\displaystyle J^s(\basereduc)}{\displaystyle \sum_{(t,\mu) \in \mathcal{P}^s} \| \dispdiscr(t,\mu) \|_2^2} \right)^{\frac{1}{2}} 
 = \left( \frac{\displaystyle\sum_{i=n_c+1}^{n_u} \lambda_i^s}{\displaystyle \sum_{i=1}^{n_u} \lambda_i^s}   \right)^{\frac{1}{2}} \, .
 %\end{array}
\end{equation}
Notice that this \textit{a priori} error estimate only provides information about the distance between the exact solution and its projection in the reduced basis for sample space $\mathcal{P}^s$. 

In the case of parametrised problem, the snapshot POD has been widely used over the years as it permits to construct an affordable approximation of $\bar{\dispdiscr}$ with only a discrete representation of the exact solution ${\dispdiscr}$. The main underlying idea is that the low-dimensional manifold of $\mathbb{R}^{n_u}$ engendered by the time and parametric dependency of the problem over space $\tilde{\mathcal{P}}$ can be captured by performing the snapshot POD transform with a relatively small number of well-chosen solution samples (see for instance \cite{kunischvolkwein2010}).

In terms of usage of the snapshot POD transform, the weights ${\basereduc^s}^T  \dispdiscr(t,\mu)$ in equation \eqref{eq:SepVariablesDiscrTime2} for $(t,\mu) \notin \mathcal{P}^s$ cannot be known in advance, as they would require the computation of the corresponding exact solution. Two different strategies can be applied to obtain them at cheap costs. The interpolation from discrete sample space $\mathcal{P}^s$ to continuous domain $\mathcal{P})$ can be done \textit{a priori} using, for instance, polynomial bases defined over $\mathcal{P})$, or \textit{a posteriori} by constructing a reduced order model (see for instance \cite{antoulassorensen2001,kunischvolkwein1999,ravindran2000}). In the latter case, the value of the weight functions are obtained at the points of interest by minimisation of problem \eqref{eq:discretized_equilibrium} projected into the space $\textrm{Im}(\basereduc^s)$ spanned by the space vectors of the snapshot POD.



\subsection{Locally uncorrelated solutions in the case of stochastic fracture}
\label{sec:Locally_uncorrelate}

\begin{figure*}[htb]
       \centering
       \includegraphics[width=0.7 \linewidth]{figures/ErrorUncorrelated}
       \caption{Definition of the lattice problem.}
       \label{fig:ErrorUncorrelated}
\end{figure*}

The expectation that a low-dimensional manifold that is relevant to the parametrised problem is correctly captured by the snapshot POD can be formalised as follows. We would like to express the fact the snapshot methodology is valid if the projection error $\nu^s$, at a certain order of the snapshot POD transform $\dispdiscr^s$, does not depend on the choice and number of solution samples, which reads
\begin{equation}
 \nu(\dispdiscr^s) - \nu(\dispdiscr^s) \leq \epsilon_{sto} \, .
\end{equation}
Of course, computing $\nu(\dispdiscr^s)$ requires the knowledge of the exact solution over the full parameter domain, which is not tractable. We instead look for the stochastic convergence of 
\begin{equation}
 \nu(\dispdiscr^s) - \tilde{\nu}(\dispdiscr^s) \, .
\end{equation}
where $\tilde{\nu}$ is the projection error of the the exact solution in $\tilde{\mathcal{P}}^s = \mathcal{P}^s \cup \tilde{\mathcal{P}}$
\begin{equation}
\tilde{\nu}(\dispdiscr^s) = \left(   \frac{\displaystyle \sum_{(t,\mu) \in \tilde{\mathcal{P}}^s}  \| \dispdiscr(t,\mu) - \bar{\dispdiscr}^s(t,\mu) \|_2^2 }{\displaystyle \sum_{(t,\mu) \in \tilde{\mathcal{P}}^s} \| \dispdiscr(t,\mu) \|_2^2} \right)^{\frac{1}{2}} 
\end{equation}

. In other words, the projection error should be independent of the choice of the samples.

However, we will see in the next section that solutions to fracture in random heterogeneous media do not necessarily reside in a manifold of small dimension, which jeopardises the application of such methods to the problem of interest.

Figure \ref{fig:ErrorUncorrelated} shows the convergence of the snapshot POD, which is usually represented by plotting the normalised error in the POD metric $\nu_{S}$ as a function of the order of the decomposition $n_c$, for different snapshots. The snapshots only differ in the number $n_\mu$ of realisations of the random distribution for which an exact solution in time has been computed.

Using only the solutions in time for the first random distribution of particles as a snapshot ($\tilde{\mathcal{P}}^h =\mu_1$), on can see that the POD converges quickly, reaching an acceptable level of error of $\nu_{S} = 10^{-3}$ at order 5. Difficulties appear when adding to this snapshot the solutions in time for a second realisation, $\tilde{\mathcal{P}}^h=\{ \mu_1, \mu_2 \}$. We find that the order of the decomposition required to reach the same level of error is doubled. As the number of realisations used to construct the snapshot increases, the same trend is observed: each new realisation requires the addition of new modes in the decomposition. As a result, it seems impossible to extract some globally correlated information from this stochastic fracture problem.


\begin{figure*}[htb]
       \centering
       \includegraphics[width=0.7 \linewidth]{figures/LocalError.pdf}
        \caption{Definition of the lattice problem.}
      \label{fig:LocalError}
\end{figure*}

However, we can show that this issue comes from very localised uncorrelated data, in the region were the different cracks propagate. To show evidences of this facts, first notice that the snapshot POD metric \eqref{eq:snapmetric} can be written as a sum of local contributions in space:
\begin{equation}
\begin{array}{ll}
J_S(\basereduc,\alpha) & \displaystyle  = \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h}  \V{\bm{\epsilon}}(t,\mu) ^T  \V{\bm{\epsilon}}(t,\mu) 
\\
& \displaystyle = \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h} \sum_{i=1}^{n_u}  \bm{\epsilon}_i(t,\mu)^2
\\
& \displaystyle
= \sum_{i=1}^{n_u} \left( \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h}   \bm{\epsilon}_i(t,\mu)^2 \right)
\end{array} \, .
\end{equation}
Let us introduce the vector $\V{\bar{\bm{\epsilon}}} \in \mathbb{R}^{n_u}$ of local contributions to the snapshot POD metric by defining its components
\begin{equation}
\label{eq:LocContr}
\bar{\bm{\epsilon}}_i =  \sqrt{ \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h} \left( \bm{\epsilon}_i(t,\mu) \right)^2 } \quad \forall \, i \in \llbracket 1, n_u\rrbracket \, .
\end{equation}
We then have the relation
\begin{equation}
\displaystyle \V{\bar{\bm{\epsilon}}}^T \V{\bar{\bm{\epsilon}}} = \sum_{i=1}^{n_u}  \bar{\bm{\epsilon}}_i^2 = \displaystyle J_S(\basereduc,\alpha) \, .
 \end{equation}
%Vector $\V{\bar{\bm{\epsilon}}}$ is normalised as follows.
%\begin{equation}
%\V{\bar{\bar{\bm{\epsilon}}}} =  \frac{\V{\bar{\bm{\epsilon}}}}{ \displaystyle  \left(   %\sum_{(t,\mu) \in \tilde{\mathcal{P}}^h} \| \dispdiscr(t,\mu) \|_2^2  \right)^\frac{1}{2}} \, .
%\end{equation}
%Hence $\V{\bar{\bar{\bm{\epsilon}}}}^T \V{\bar{\bar{\bm{\epsilon}}}} = \nu_S^2$
The vector of local contributions to the snapshot POD metric $\V{{\bar{\bm{\epsilon}}}}$ is represented in figure \ref{fig:LocalError} (top figure). Solutions in time corresponding to 10 parameter samples have been used as a snapshot in this case. The snapshot POD is truncated at order 12, which leads to an error $\nu_S = 4.3 \times 10^{-2}$. It clearly appears that the major contributors to the snapshot POD metric are localised in a narrow region: the process zone.

%\begin{figure*}[htb]
%       \centering
%       \includegraphics[width=0.7 \linewidth]{figures/ErrorUncorrelated2}
%       \caption{Definition of the lattice problem.}
%       \label{fig:ErrorUncorrelated2}
%\end{figure*}



\subsection{Tools for the enhancement the convergence of POD transforms}



The idea of the weighted POD is to increase the convergence rate of the decomposition by giving less importance to uncorrelated data in space or time. A typical Weighted version of the POD metric \eqref{eq:MetricPOD} would read
\begin{equation}
\label{eq:WeightedPODCont}
J_W(\basereduc,\alpha) = \int_{(t,\mu) \in \tilde{\mathcal{P}}} \| \V{\bm{\epsilon}} (t,\mu) \|_{\M{\mathbf{L}}} \Phi(t,\mu)  \, dt \, d\mu \ ,
\end{equation}
Equivalently in the case of the snapshot POD applied to the considered stochastic problem of evolution, functional \eqref{eq:snapmetric} is replaced by
\begin{equation}
\label{eq:WeightedPOD}
J_{SW}(\basereduc,\alpha) = \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h} \| \V{\bm{\epsilon}}(t,\mu) \|_{\M{\mathbf{L}}}^2 \ \Phi(t,\mu) \, .
\end{equation} 
In equations \eqref{eq:WeightedPODCont} and \eqref{eq:WeightedPOD}, $\Phi \in \mathcal{F}(\tilde{\mathcal{P}})$ is a scalar time/parameter weight function, and $\M{\mathbf{L}} \in \mathbb{R}^{n_u} \times \mathbb{R}^{n_u}$ is a diagonal operator with strictly positive entries (i.e.: the space weights). The weighted euclidean norm $\| \, . \, \|_{\M{\mathbf{L}}}$ in $\mathbb{R}^{n_u}$ is defined by
 \begin{equation}
 \| \X \|_{\M{\mathbf{L}}} = \sqrt{\X^T \M{\mathbf{L}} \, \X} \, ,
 \end{equation}
 for arbitrary vector $\X \in \mathbb{R}^{n_u}$.


 %The idea of the weighted POD is to increase the convergence rate of the decomposition by giving less weight to uncorrelated data in space or time. A typical Weighted version of the POD metric \eqref{eq:MetricPOD} would read
 %\begin{equation}
 %\ label{eq:WeightedPODCont}
% d_W(\dispdiscr,\bar{\dispdiscr}) = \int_{t \in \mathcal{\tau}} \| \V{\bm{\epsilon}} (t,\mu) \|_{\M{\mathbf{L}}_t(t)}^2  \, dt \ .
 %\end{equation}
 %where $\V{\bm{\epsilon}} = \dispdiscr - \bar{\dispdiscr}$ over time domain $\tau$. Equivalently in the case of the snapshot POD applied to the considered stochastic problem of evolution, functional \eqref{eq:snapPODmetric} is replaced by
 %\begin{equation}
 %\label{eq:WeightedPOD}
 %J_{SW}(\basereduc,\alpha) = \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h} \| \V{\bm{\epsilon}}(t_n,\mu) \|_{\M{\mathbf{L}}_p(t,\mu)}^2  \, .
 %\end{equation} 
 %In equations \eqref{eq:WeightedPODCont} and \eqref{eq:WeightedPOD}, $\M{\mathbf{L}}_t(t)$ and $\M{\mathbf{L}}_p(t,\mu)$ are diagonal operators with strictly positive entries (i.e.: the space weights). The weighted euclidean norm $\| \, . \, \|_{\M{\mathbf{L}}}$ in $\mathbb{R}^{n_u}$ is defined by
 %\begin{equation}
 %\| \X \|_{\M{\mathbf{L}}} = \sqrt{\X^T \M{\mathbf{L}} \, \X} \, ,
 %\end{equation}
 
 In our case, we would intuitively like the entries of $\M{\mathbf{L}}$ that correspond to the part of the domain where the snapshot data is not correlated to be small. How small these weights should be is obviously difficult to address. Weights that are too small would lead to numerical ill-posedness of the POD minimisation problem, weights that are too large would pollute the results in the zones where the snapshot data is correlated. We propose to extend the idea of weighted POD transforms by performing a POD-type decomposition of the data corresponding to only a part of the degrees of freedom. 
 
 This set of degrees of freedom, called spatial domain of validity of the POD transform, are the one for which the local contributions to the POD metric \ref{eq:LocContr} is small enough.In turn, obtaining these local contributions require the knowledge of an initial POD transform. Hence, we arrive at the idea of an iterative process to find an optimal POD-type decomposition associated with a domain of validity, which is in substance what is proposed in the following section.
 
 
 % Intuitively, the idea is to state that the decomposition is only valid in the region of the domain were the local contributions to this metric are sufficiently small (figure \ref{fig:LocalError} bottom). However, the evaluation the POD functional in the non-correlated zones can ``pollute'' the decomposition. In other words, the decomposition is not optimal in the spatial domain of validity.



%--------------------------------------------------------

\section{Progressive Restricted POD for locally uncorrelated solutions}

%--------------------------------------------------------

\subsection{A limit case of the Weighted POD: the Restricted POD}
\label{sec:RestrictedPOD}

The proposed restricted POD performs a classical POD of the spatial components of the snapshot samples corresponding to a high level of correlation (i.e. the process zone). These components will be denoted by superscript $^{(r)}$. This transform being computed, the POD-type decomposition of the complementary components, denoted by $^{(f)}$ are obtained by minimisation of a global metric.

Formally, let us decompose the euclidean space $\mathbb{R}^{n_u}$ as a product of two spaces: $ \mathbb{R}^{n_u} = \mathbb{R}^{n_r} \times \mathbb{R}^{n_f}$. Any vector $\X \in \mathbb{R}^{n_u}$ will be decomposed as follows
\begin{equation}
\X = ( \X^{(r)}, \X^{(f)} ) \in \mathbb{R}^{n_r} \times \mathbb{R}^{n_f} \, .
\end{equation}
We introduce the boolean restriction operators $\M{\mathbf{E}}^{(r)} \in  \{ 0 , 1 \}^{n_r} \times \{ 0 , 1 \}^{n_u}$ and $\M{\mathbf{E}}^{(f)} \in \{ 0 , 1 \}^{n_f} \times \{ 0 , 1 \}^{n_u}$ such that
\begin{equation}
\begin{array}{c}
\displaystyle \X^{(r)} = \M{\mathbf{E}}^{(r)} \X \\
\displaystyle \X^{(f)} = \M{\mathbf{E}}^{(f)} \X
\end{array} \, ,
\end{equation}
Hence, $\X \in \mathbb{R}^{n_u}$ can be written as a sum of two contributions
\begin{equation}
\X  = {\M{\mathbf{E}}^{(r)}}^T \X^{(r)} + {\M{\mathbf{E}}^{(f)}}^T \X^{(f)} \, .
\end{equation}
%\begin{equation}
%\begin{array}{ll}
%\X & \displaystyle  = {\M{\mathbf{E}}^{(r)}}^T \X^{(r)} + {\M{\mathbf{E}}^{(f)}} \X^{(f)}  \\
% & \displaystyle = {\M{\mathbf{P}}^{(r)}} \X + {\M{\mathbf{P}}^{(f)}} \X 
%\end{array} \, ,
%\end{equation}
%where we have introduced the projectors ${\M{\mathbf{P}}^{(r)}} = {\M{\mathbf{E}}^{(r)}}^T {\M{\mathbf{E}}^{(r)}}$ and ${\M{\mathbf{P}}^{(f)}} = {\M{\mathbf{E}}^{(f)}}^T {\M{\mathbf{E}}^{(f)}}$.

The Restricted POD looks for a decomposition of the Snapshots in the form 
\begin{equation}
\label{eq:SepVariablesDiscrTimeRestr}
\begin{array}{rcl}
\displaystyle  \bar{\V{\mathbf{\mathbf{S}}}}  : \  \tilde{\mathcal{P}}^h & \displaystyle \rightarrow & \displaystyle \mathbb{R}^{n_u} 
\\ \displaystyle
\displaystyle (t,\mu) &  \mapsto & \displaystyle \left(  {\M{\mathbf{E}}^{(r)}}^T \basereduc^{(r)} + {\M{\mathbf{E}}^{(f)}}^T \basereduc^{(f)} \right) \coeffreduc(t,\mu)  \, .
\end{array}
\end{equation}

As in the classical snapshot POD, $\bar{\V{\mathbf{\mathbf{S}}}}$ minimises a distance with respect to $\V{\mathbf{\mathbf{S}}}$. The restricted decomposition minimises functional
\begin{equation}
J_{SR} (  \basereduc^{(r)} , \basereduc^{(f)}, \coeffreduc )  = J_{SR}^{(r)} (  \basereduc^{(r)}, \coeffreduc ) + J_{SR}^{(f)} ( {\basereduc^{(f)}} ) \, ,
\end{equation}
where
\begin{equation}
 J_{SR}^{(r)} ( \basereduc^{(r)},\coeffreduc )  = \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h} \|  \V{\bm{\epsilon}}^{(r)}(t,\mu) \|_2^2 \, ,
\end{equation}
where function $\V{\bm{\epsilon}}^{(r)} \in \mathcal{V}^{h,(r)}$ is defined by $\V{\bm{\epsilon}}^{(r)} = {\M{\mathbf{E}}^{(r)}}\V{\mathbf{\mathbf{S}}} -  \basereduc^{(r)} \coeffreduc$,
and
\begin{equation}
J_{SR}^{(f)} ( {\basereduc^{(f)}} ) = \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h} \|  \V{\bm{\epsilon}}(t,\mu) \|_2^2 \, .
\end{equation}
The optimisation is constrained by the orthonormality condition
\begin{equation}
{\basereduc^{(r)}}^T {\basereduc^{(r)}} = \M{\mathbf{I}}_d
\end{equation}

The constrained minimisation of $J_{SR}^{(r)}$ with respect to $(\basereduc^{(r)},\coeffreduc)$ is a classical POD problem in $\mathbb{R}^{n_r}$ and leads to the complete determination of ${\M{\mathbf{E}}^{(r)}} \bar{\V{\mathbf{\mathbf{S}}}}$:
\begin{itemize}
\item  $( \V{\mathbf{C}}_i^{(r)} )_{i \in \llbracket 1, n_c \rrbracket}$ are the eigenvectors of $\displaystyle \bar{\M{\mathbf{H}}}^h = \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h} {\M{\mathbf{E}}^{(r)}} \dispdiscr(t,\mu) \, \dispdiscr(t,\mu)^T {\M{\mathbf{E}}^{(r)}}^{T}$ associated to its largest $n_c$ eigenvalues $(\bar{\lambda}_i)_{i \in \llbracket 1, n_c \rrbracket}$.
\item $\coeffreduc =  {\basereduc^{(r)}}^T  \, \M{\mathbf{E}}^{(r)} \bar{\V{\mathbf{\mathbf{S}}}} $
\end{itemize}


The minimisation of $J_{SR}^{(f)}$ with respect to $\basereduc^{f}$, knowing the previously defined restricted POD decomposition ${\M{\mathbf{E}}^{(r)}} \bar{\V{\mathbf{\mathbf{S}}}}$, leads to the determination of restricted POD transform $\basereduc^{f}$:
\begin{equation}
\basereduc^{(f)}  =  \M{\mathbf{G}} \, \M {\bm \alpha}^{-1} \, ,
\end{equation}
where $\displaystyle  \M{\mathbf{G}} = \left( {\M{\mathbf{E}}^{(f)}} \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h}  \dispdiscr(t,\mu) \,  \coeffreduc(t,\mu)^{T} \right)$ 
and $\displaystyle \M {\bm \alpha} = \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h} \coeffreduc(t,\mu) \, \coeffreduc(t,\mu)^{T} $



The truncation error for the restricted snapshot POD of order $n_c$ is:
\begin{equation}
J_{SR}^{(r)}(\basereduc^{(r)},\coeffreduc) = \sum_{i=n_c+1}^{n_u} \lambda_i
\end{equation}

As for the classical snapshot POD, we define the normalised truncation error:
\begin{equation}
\displaystyle  \nu_{SR}^{(r)}  \displaystyle  = \left( \frac{\displaystyle\sum_{i=n_c+1}^{n_u} \lambda_i}{\displaystyle \sum_{i=1}^{n_u} \lambda_i}   \right)^{\frac{1}{2}} 
\end{equation}

The value of functional $J_{SR}^{(f)}$ provides an error estimate for ${\M{\mathbf{E}}^{(f)}} \bar{\V{\mathbf{\mathbf{S}}}}$. However, this is not of much use as $J_{SR}^{(f)}$ will measure a projection of snapshot data that cannot be approximated in a low-dimensional subspace of $\mathbb{R}^{n_f}$ onto reduced space of low dimension $\textrm{Im}(\basereduc^{(f)})$.

Now that the restricted POD is defined, we need to be able to obtain the splitting between $^{(f)}$ and $^{(r)}$ spatial components. This is what is proposed next.


\subsection{Progressive Weighted / Restricted POD}
\label{sec:ProgressivePOD}

The general goal of this section is to look for a decomposition of the solution as a sum of products of functions of separate variables, and, at the same time, for the associated weighted or restricted POD metric that has to be minimised. The proposition holds for any weighted-type POD transform, but we apply it directly to the case of the restricted POD.

The optimisation problem of interest can be formulated as the search of a decomposition $\bar{\V{\mathbf{\mathbf{S}}}}$ of type \eqref{eq:SepVariablesDiscrTimeRestr}, and an associated restricted metric $J_{SR}$ with parameter $\left( {\M{\mathbf{E}}^{(r)}} \right)$ such that $\bar{\V{\mathbf{\mathbf{S}}}}$ minimises $J_{SR}$ and the convergence of error criterion $\nu_{SR}^{(r)}$ with $n_c$ is sufficiently fast.

A class of progressive POD algorithms is proposed below to obtain a solution to such a problem.
\begin{enumerate}
\item Initialise the algorithm with a POD functional $J_{SR}^{0}$, by choosing initial parameter $ {\M{\mathbf{E}}^{(r),0}} $, and set $i=1$
\item For functional $J_{SR}^{i-1}$, compute a POD-type decomposition $\V{\mathbf{\bar{\mathbf{S}}}}^{i}$ of order $n_c^{i}$, such that the  truncation error $J_{SR}^{(r),i-1}(\M{\mathbf{E}}^{(r),i-1} \basereduc^{i},\coeffreduc^{i})$ is sufficiently low.
\item Update parameters $\M{\mathbf{E}}^{(r),i}$ of functional $J_{SR}^{i}$ so that for a fixed decomposition $\V{\mathbf{\bar{\mathbf{S}}}}^{i}$, the normalised error in the POD metric $J_{SR}^{(r),i}(\M{\mathbf{E}}^{(r),i} \basereduc^{i},\coeffreduc^{i})$ decreases sufficiently with respect to $J_{SR}^{(r),i-1}(\M{\mathbf{E}}^{(r),i-1} \basereduc^{i},\coeffreduc^{i})$.
\item Evaluate the convergence of the algorithm. If convergence is not achieved, set $i \leftarrow i+1$ and go to back to step 2.
\end{enumerate}

Choices are needed to fully define each of these four stages. In the following sections, we particularise the previous generic algorithm to the case of the targeted problem of stochastic fracture.


\subsubsection{Initialisation (Step 1)} 

Let us first make the natural choice of a classical POD metric for the initialisation $J_{SR}^{0} = J_{S}$, which corresponds to parameter ${\M{\mathbf{E}}^{(r),0}} = \M{\mathbf{I}}_d$.

\subsubsection{Selection of the Restricted POD modes (Step 2)}

\begin{figure*}[htb]
       \centering
       \includegraphics[width=0.7 \linewidth]{figures/ErrorNModesPourReduc}
       \caption{Definition of the lattice problem.}
       \label{fig:ErrorNModesPourReduc}
\end{figure*}

The definition of step 2 of the progressive restricted POD requires more insight of the problem that is at sack here. Let us take a look at figure \ref{fig:ErrorNModesPourReduc}. This graph displays convergence curves of the restricted POD $\nu_{SR}^{(r)}$, in the plane defined by the axis labelled $\nu_{SR}^{(r)}$ and $n_c$, as a function of the order of the decomposition, for different parameters of the restricted metric (along the axis labelled $P_{Red}$). $P_{Red}$ is the percentage of spatial components for which the eigenvalue problem of the restricted POD is computed, namely the number of non-zero entries of $\M{\mathbf{E}}^{(r)}$ divided by $n_u$, and multiplied by 100.
For an easier reading, the projection of this figure in planes $(\nu_{SR}^{(r)},n_c)$ and $(\nu_{SR}^{(r)},P_{Red})$ are given in figure \ref{fig:ErrorNModesPourReduc2} and \ref{fig:ErrorNModesPourReduc3} respectively. This result is obtained by taking as snapshot the solutions in time that correspond to 10 realisations of the stochastic distributions of material properties, $\mathbf{P}^h=\{ \mu_1, \, ... \, \mu_{10} \}$.

The main characteristic that we want to point out at this stage is that two regimes of convergence of $\nu_{SR}^{(r)}$ as a function of $n_c$ can be observed. A very fast convergence for a decomposition of low order, and a slower convergence in the later regime. The idea is to select only the modes corresponding to this first regime, as adding further modes does not significantly improve the approximation. Following this principle, picking up the desired number of modes by sight seems relatively easy (6 for the bottom curve in figure \ref{fig:ErrorNModesPourReduc2} for instance), but making the process automatic is not a trivial task.

In a log scale for the error in the POD metric, the observed two different regimes of convergence are qualitatively close to linear. We propose to fit two straight lines to approximate the convergence curve, and set the optimal number of modes as the intersection of these two lines (figure \ref{fig:LeastSquaresModes}). 

\begin{figure*}[p]
       \centering
       \includegraphics[width=0.7 \linewidth]{figures/ErrorNModesPourReduc2}
       \caption{Definition of the lattice problem.}
       \label{fig:ErrorNModesPourReduc2}
\end{figure*}

\begin{figure*}[p]
       \centering
       \includegraphics[width=0.7 \linewidth]{figures/ErrorNModesPourReduc3}
       \caption{Definition of the lattice problem.}
       \label{fig:ErrorNModesPourReduc3}
\end{figure*}

Let us develop this idea. We call $\nu^c \in \mathcal{C}^0([{n_c}_{min},{n_c}_{max}])$ the piecewise linear interpolation of the convergence curve (i.e. linear interpolation between two successive points of the convergence curve).
$\bar{\nu}^c \in \mathcal{C}^0([{n_c}_{min},{n_c}_{max}])$ denotes its approximation by two straight lines.
\begin{equation}
\begin{array}{rcl}
\bar{\nu}^c: \quad [{n_c}_{min},{n_c}_{max}] & \rightarrow & \mathbb{R^+} \\
n^c_c & \mapsto & \left\{
						\begin{array}{l}
						a^- n^c_c + b^- \\ \quad \textrm{if } n^c_c<n^c_{c,I}
						\\
						a^+ n^c_c + b^+ \\ \quad \textrm{if } n^c_c>n^c_{c,I} 
						\end{array}
						\right.  .
\end{array}
\end{equation}
$a = \{a^-,b^-,a^+,b^+ \}$ are the parameters of the approximate convergence curve, while $n^c_{c,I} $ is the abscissa of the intersection point of the two straight lines defining this approximation. The least-square functional that we minimise to fit the approximation to the convergence curve is:
\begin{equation}
\begin{array}{ll}
\displaystyle J_{n_c}(a,n^c_{c,I}) & \displaystyle = \int_{{n_c}_{min}}^{n^c_{c,I}} (\nu^c-\bar{\nu}^c)^2 \, dn^c_c \\
& \displaystyle + \int_{n^c_{c,I}}^{{n_c}_{max}} (\nu^c-\bar{\nu}^c)^2 \, dn^c_c 
\end{array} \, ,
\end{equation}
We also enforce continuity of the approximation $\bar{\nu}^c$:
\begin{equation}
n^c_{c,I} = \frac{b^+ - b^-}{a^- - a^+} \, ,
\end{equation}

This problem can be reformulated as a fixed point for the constraint equation by observing that solution $n^c_{c,I}$ is such that
\begin{equation}
n^c_{c,I} = \frac{b^+(n^c_{c,I}) - b^-(n^c_{c,I})}{a^-(n^c_{c,I}) - a^+(n^c_{c,I})} \, ,
\end{equation}
where $a$ minimises $J_{n_c}(a,n^c_{c,I})$.

Hence we can easily solve this problem by the following fixed-point algorithm:
\begin{enumerate}
\item $n^{c,0}_{c,I} = \displaystyle \frac{ {{n_c}_{max}} - {{n_c}_{min}} }{ 2 }$ and set $l=1$
\item $a^{l} = \underset{a^\star}{\textrm{argmin}} (J_{n_c}(a^\star,n^{c,l}_{c,I})$, which yields a linear system in $a^l$.
\item $n^{c,l}_{c,I} = \displaystyle \frac{b^{+,l} - b^{-,l}}{a^{-,l} - a^{+,l}}$
\item if $\frac{|n^{c,l}_{c,I} - n^{c,l-1}_{c,I}|}{n^{c,l-1}_{c,I}} > 10^{-2}$ set $l \leftarrow l+1$ and go back to step 2, else set the final number of selected modes $n_c$ for the decomposition $\bar{\V{\mathbf{\mathbf{S}}}}$, $n_c = \textrm{floor} (n^{c,l}_{c,I}+1) $.
\end{enumerate}

A result of this technique is given in figure \ref{fig:LeastSquaresModes}, for the initial metric of the restricted POD $J_{SR}^{0}$. The black curve in figures \ref{fig:ErrorNModesPourReduc}, \ref{fig:ErrorNModesPourReduc2} and \ref{fig:ErrorNModesPourReduc3} shows the number of selected modes, and the associated normalised error in the POD metric, that are selected when applying this methodology at successive step of the progressive POD algorithm. One can see that we successfully manage to isolate the regime of fast convergence of the restricted POD.

\begin{figure}[htb]
       \centering
       \includegraphics[width=0.7 \linewidth]{figures/LeastSquaresModes}
       \caption{Definition of the lattice problem.}
       \label{fig:LeastSquaresModes}
\end{figure}


\subsubsection{Update of the metric (Step 3)}

Recall the expression of the POD functional as a sum of local contributions in space, that we can apply to the restricted POD:
\begin{equation}
\begin{array}{l}
\displaystyle J_{SR}^{(r)}(\basereduc^{(r),i},\alpha^i) ={\bm{\bar{\epsilon}}^{(r)}} \cdot {\bm{\bar{\epsilon}}^{(r)}} 
\\
\displaystyle \textrm{with} \ \bm{\bar{\epsilon}}_i =  \sqrt{ \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h} \left( \bm{\epsilon}_i^{(r)}(t,\mu) \right)^2 } \quad \forall i \in \llbracket 1, n_r^i \rrbracket \, .
%\label{eq:LocContr}
%\bar{\bm{\epsilon}}_i =  \sqrt{ \sum_{(t,\mu) \in \tilde{\mathcal{P}}^h} \left( \bm{\epsilon}_i(t,\mu) \right)^2 } \quad \forall \, i \in \llbracket 1, n_u\rrbracket \, .
 \end{array}
 \end{equation}
Function $\bm{\bar{\epsilon}}$ is here fixed as the decomposition has been calculated at Step 2 of the Progressive POD algorithm. 

We propose to remove the maximum local contribution from the $^{r}$ degrees of freedom. Let us denote by $\displaystyle i_{max}=\text{argmin}_{ \, i \in \llbracket 1, n_r^i \rrbracket}  \bm{\epsilon}_i^2$ the index of this maximum local contribution. The updated extractor $\M{\mathbf{E}}^{(r),i} \in \mathbb{R}^{n_r^i \times n_u}$, where $n_r^i = n_r^{i-1} - 1$, reads
\begin{equation}
\begin{array}{ll}
\displaystyle \forall \, j \in \llbracket 1, n_u\rrbracket , & \\
\M{\mathbf{E}}^{(r),i}_{i,j} = \M{\mathbf{E}}^{(r),i-1}_{i,j} & \ \forall \, i \in \llbracket 1, n_r^{i-1} \rrbracket \, | \, i<i_{max} 
\\ \displaystyle
\M{\mathbf{E}}^{(r),i}_{i,j} = \M{\mathbf{E}}^{(r),i-1}_{i+1,j} & \  \forall \, i \in \llbracket 1, n_r^{i-1} \rrbracket \, | \, i>i_{max} \, .
\end{array}  
\end{equation}
The second updated extractor $\M{\mathbf{E}}^{(f),i} \in \mathbb{R}^{n_f^i \times n_u}$ , where $n_f^i = n_u - n_r^i$, is then given by the definition of such an extractor, and the property:
\begin{equation}
{\M{\mathbf{E}}^{(f),i}}^T \M{\mathbf{E}}^{(f),i} = \mathbf{\M{I}}_d - {\M{\mathbf{E}}^{(r),i}}^T \M{\mathbf{E}}^{(r),i} \, .
\end{equation}

In practice, one can choose to move more than one of the space components from $^{(r)}$ to $^{(f)}$ at a time to fasten the Progressive POD algorithm. In our test cases, we remove all the space components corresponding to nodes situated in a sphere of ray two times the length of a lattice element, entered on the node carrying the largest contribution to the POD metric. Provided that this step is not too large, it does not affect the results significantly.


\subsubsection{Convergence of the Progressive Restricted POD (Step 4)}


\begin{figure}[htb]
       \centering
       \includegraphics[width=0.7 \linewidth]{figures/LeastSquaresPourReduc}
       \caption{Definition of the lattice problem.}
       \label{fig:LeastSquaresPourReduc}
\end{figure}

A similar trend as the one observed for Step 2 is observed here. I clearly appears in figures \ref{fig:ErrorNModesPourReduc} and \ref{fig:ErrorNModesPourReduc3} that the normalised error in the POD metric, for a given number of selected modes, decreases in a fast manner at the very first iterations of the Progressive POD (small amount of space components remove from the POD calculation), and then tends to stagnate, or decreases more slowly. We apply the same procedure described for Step 2 to stop the updates of the POD metric. A typical fitting is displayed in figure \ref{fig:LeastSquaresPourReduc}, where a fixed number of modes $n_c = 3$ is considered at Step 2 for the whole simulation.

The considered solution of the Progressive POD is at the intersection of the black in blue lines in figures \ref{fig:ErrorNModesPourReduc}, \ref{fig:ErrorNModesPourReduc2} and \ref{fig:ErrorNModesPourReduc3}. We find in this example an optimal number of modes $n_c = 6$ and a domain of validity of the Restricted POD equal to 88 \% of the number of initial space components.
